Fine Tuning without Catastrophic Forgetting via Selective Low Rank Adaptation

Adapting deep learning models to new domains often requires computationally intensive retraining and risks catastrophic forgetting. While fine-tuning enables domain-specific adaptation, it can reduce robustness to distribution shifts, impacting out-of-distribution (OOD) performance. Pre-trained zero-shot models like CLIP offer strong generalization but may suffer degraded robustness after fine-tuning. Building on Task Adaptive Parameter Sharing (TAPS), we propose a simple yet effective extension as a parameter-efficient fine-tuning (PEFT) method, using an indicator function to selectively activate Low-Rank Adaptation (LoRA) blocks. Our approach minimizes knowledge loss, retains its generalization strengths under domain shifts, and significantly reduces computational costs compared to traditional fine-tuning. We demonstrate that effective fine-tuning can be achieved with as few as 5\% of active blocks, substantially improving efficiency. Evaluations on pre-trained models such as CLIP and DINO-ViT demonstrate our method's broad applicability and effectiveness in maintaining performance and knowledge retention.

==> sections/9_apendix_tmp.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary


\iffalse
\section{Related Papers}
\paragraph{Catastrophic Forgetting.} 

\begin{itemize}
    \item \href{https://arxiv.org/pdf/2403.06398}{On the Diminishing Returns of Width for Continual Learning, ICML, 2024}
    \item \href{https://proceedings.mlr.press/v162/mirzadeh22a.html}{Wide Neural Networks Forget Less Catastrophically, ICML, 2022}
    \item \href{https://openreview.net/forum?id=GhVS8_yPeEa}{Effect of scale on catastrophic forgetting in neural networks, ICLR, 2022}
    \item \href{https://arxiv.org/abs/2405.18069}{An Empirical Analysis of Forgetting in Pre-trained Models with Incremental Low-Rank Updates, Arxiv, 2024}
    \item \href{https://arxiv.org/pdf/2207.09074}{Incremental Task Learning with
Incremental Rank Updates, ECCV, 2022}
    \item \href{https://arxiv.org/pdf/2306.01904}{Overcoming the Stability Gap in Continual Learning, TMLR, 2024}
    \item \href{https://openaccess.thecvf.com/content/ICCV2023/papers/Gao_A_Unified_Continual_Learning_Framework_with_General_Parameter-Efficient_Tuning_ICCV_2023_paper.pdf}{A Unified Continual Learning Framework with General Parameter-Efficient Tuning, ICCV, 2023}
    \item \href{https://arxiv.org/pdf/2403.05175v1}{Continual Learning and Catastrophic Forgetting}
    \item \href{https://openaccess.thecvf.com/content/CVPR2022/papers/Wang_Learning_To_Prompt_for_Continual_Learning_CVPR_2022_paper.pdf}{Learning to Prompt for Continual Learning}
    \item \href{https://proceedings.mlr.press/v80/serra18a/serra18a.pdf}{Overcoming Catastrophic Forgetting with Hard Attention to the Task}
    \item \href{https://arxiv.org/pdf/2304.04158}{Does Continual Learning Equally Forget All Parameters?}
    \item \href{https://arxiv.org/abs/2402.07410}{A Closer Look at the Robustness of Contrastive
Language-Image Pre-Training (CLIP)https://arxiv.org/abs/2402.07410}
\end{itemize}


\paragraph{Others.}

\begin{itemize}
    \item \href{https://arxiv.org/pdf/1701.08734}{PathNet: Evolution Channels Gradient Descent in Super
Neural Networks}
    \item \href{https://arxiv.org/pdf/2004.00070}{Conditional Channel Gated Networks for Task-Aware Continual Learning}
    \item \href{https://arxiv.org/pdf/2310.16226}{TiC-CLIP: Continual Training of CLIP Models}
    \item \href{https://arxiv.org/pdf/2303.06628}{Preventing Zero-Shot Transfer Degradation in Continual Learning of
Vision-Language Models}
    \href{Overcoming Domain Limitations in Open-vocabulary Segmentation}{https://arxiv.org/pdf/2410.11536}
    \href{Are Straight-Through gradients and Soft-Thresholding all you need for Sparse Training?}{https://www.semanticscholar.org/paper/Are-Straight-Through-gradients-and-all-you-need-for-Vanderschueren-Vleeschouwer/e2a06471cd317ff426c1cc79c0139cd12f699f00}
\end{itemize}


\section{Tasks} \begin{itemize} 
\item Finetuning and evaluating the Florence model with different ranks (4, 8, 16, 32, 64, 128, and 256) using LoRA and DoRA. 
\item For the Florence model, we can use the nuScenes dataset for in-distribution evaluation, and MS-COCO and Flickr for assessing zero-shot capability. \item Ensure access to the model weights required for Section 5.2. \item Decide on the appropriate function to use for Section 5.4. \end{itemize}


\begin{figure*}
     \centering
     \includegraphics[width=\linewidth]{figures/clip_lora_hinge.pdf}
     %\vspace{-3pt}
     \vspace{-0.7cm}
     \caption{.}
     \label{fig:clip}
    \vspace{-0.4cm}
\end{figure*}
\fi
